Converting BPMN Diagrams to Privacy Calculus

The ecosystem of Privacy Calculus is a formal framework for privacy comprising (a) the Privacy Calculus, a Turing-complete language of message-exchanging processes based on the pi-calculus, (b) a privacy policy language, and (c) a type checker that checks adherence of Privacy Calculus terms to privacy policies. BPMN is a standard for the graphical description of business processes which aims to be understandable by all business users, from those with no technical background to those implementing software. This paper presents how (a subset of) BPMN diagrams can be converted to Privacy Calculus terms, in the hope that it will serve as a small piece of larger workflows for building privacy-preserving software. The conversion is described mathematically in the paper, but has also been implemented as a software tool.

==> eptcsdata.tex <==
\providecommand{\firstpage}{53}
\providecommand{\publicationstatus}{M. Marin, L. Leu\c{s}tean (Eds.):\\ 
8th Symposium on Working Formal Methods (FROM 2024)\\
EPTCS 410, 2024, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.410.4}{10.4204/EPTCS.410.4}}
\pdfoutput=1

